Red Carpet to Fight Club: Partially-supervised Domain Transfer for Face Recognition in Violent Videos

In many real-world problems, there is typically a large discrepancy between the characteristics of data used in training versus deployment. A prime example is the analysis of aggression videos: in a criminal incidence, typically suspects need to be identified based on their clean portrait-like photos, instead of their prior video recordings. This results in three major challenges; large domain discrepancy between violence videos and ID-photos, the lack of video examples for most individuals and limited training data availability. To mimic such scenarios, we formulate a realistic domain-transfer problem, where the goal is to transfer the recognition model trained on clean posed images to the target domain of violent videos, where training videos are available only for a subset of subjects. To this end, we introduce the WildestFaces dataset, tailored to study cross-domain recognition under a variety of adverse conditions. We divide the task of transferring a recognition model from the domain of clean images to the violent videos into two sub-problems and tackle them using (i) stacked affine-transforms for classifier-transfer, (ii) attention-driven pooling for temporal-adaptation. We additionally formulate a self-attention based model for domain-transfer. We establish a rigorous evaluation protocol for this clean-to-violent recognition task, and present a detailed analysis of the proposed dataset and the methods. Our experiments highlight the unique challenges introduced by the WildestFaces dataset and the advantages of the proposed approach.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

%\twocolumn[{%
%\renewcommand\twocolumn[1][]{#1}%
\begin{figure*}
    %\vspace{-1cm}
    \begin{center}
        \centering
        \includegraphics[width=.95\textwidth]{figures/mainfigure_v2.pdf}
        % https://docs.google.com/drawings/d/1krBKcodnRy-lCK7WzuJIkNFTXtYnq73fuE7KFmu9DkM/edit?usp=sharing
        %\vspace{-2mm}
        \caption{Our focus is the problem of face recognition in the {\em wildest} video settings by transfering recognition models trained on clean, portrait-like images. We propose the WildestFaces dataset that selectively contains videos of violent scenes from movies, together with the clean {\em red-carpet} images of the corresponding actors. Importantly, video training examples are made available only for a subset of the actors, which leads to a challenging partially-supervised domain transfer problem.\label{fig:mainfigure}}
    \end{center}
    \vspace{-6mm}
\end{figure*}
% Also see: https://docs.google.com/presentation/d/1c5Hlgi8k4WL6F2lHyuFUAodrB1vPGtZax8ohEqF0mHw/edit#slide=id.p
%}]


%Recognition of faces have a wide range of application areas, from surveillance and security systems to consumer products and more. Accordingly, 
A plethora of studies have focused on face recognition in computer vision literature.  Compared to
the pioneering works \cite{turk1991face,ahonen2006face,xie2010fusing,edwards1998face, wright2009robust,wiskott1997face}, face recognition models that benefit from deep learning-based techniques and concentrate on better
formulation of distance metric optimization raised the bar~\cite{schroff2015facenet,taigman2014deepface,parkhi2015deep,wen2016discriminative,sun2013hybrid,sun2014deep,sun2015deepid3,deng2019arcface,zheng2018ring,wang2018cosface}. There has been interest in using additional data (in the form of unlabeled  \cite{zhan2018consensus,coelho2018face} or synthetic data \cite{zhao2017dual}), class-balancing \cite{yin2019feature}	and noisy-data handling \cite{hu2019noise} to improve face recognition accuracy as well. In addition to face recognition in still images,
video-based face recognition studies have also emerged (see  \cite{ding2016comprehensive} for a recent survey). Ranging
from local feature-based methods~\cite{li2013probabilistic,parkhi2014compact,li2014eigen} to manifolds
\cite{huang2015log} and metric learning~\cite{cheng2018duplex,huang2017cross,goswami2017face}, recent studies have
focused on finding informative frames in image sets \cite{goswami2014mdlface} and finding efficient and fast ways of
feature aggregation~\cite{chowdhury2016one,yang2017neural,rao2017learning,rao2017attention}. 

Most of these studies concentrate their effort on relatively easier cases of recognition, where the faces are seen under
good lighting conditions and are mostly stable with relatively orthogonal viewpoints. On the contrary, face recognition
in the ``wildest'' demands more than that. Especially, people engaging in criminal activities such as fighting or
disputes, are likely to expose a much diverse set of facial expressions/poses. The people in these activities are also
likely to move fast, causing the recorded video footage to have significant amount of blur and occlusion. What is even
more challenging is that, these people may not necessarily have prior criminal records, therefore may not have recorded
\textit{``fight scene footage's''}. They may only have \textit{``clean''} images, such as passport or Facebook-type of
photos, that can be used for identification. %Similarly, scuffle and fight scenes in multimedia archives arguably posses the hardest challenges for automated person indexing, and in most practical large-scale scenarios, only a fraction of such scenes can be annotated to obtain video training samples.

In this paper, we focus on the problem of face recognition in such ``wildest'' scenarios. 
% where not all target subjects may have recorded footages of violence, but only clean images. 
In order to facilitate research in this direction, we propose a new dataset, referred to as {\em WildestFaces}. This dataset
consists of clips with adverse effects at their extreme, and auxiliary clean facial images of the corresponding people.
The videos are collected by manually finding violent scenes in movies of predetermined actors\footnote{We use {\em
actor} as a gender-neutral term, following the modern practice.}, and the clean images are collected from IMDB\footnote{www.imdb.com} and similar websites. The task is depicted in
Figure~\ref{fig:mainfigure} with example images from the dataset. 
The training set provides clean still images of
all people and violent videos of only a subset of people. The test set, however, contains novel videos of all people.
This setup resembles to that of \textit{generalized zero-shot learning (GZSL)}~\cite{xian2017zero,chao16gzsl}, where there are both seen and unseen classes in testing. We define an evaluation protocol that explicitly measures the success at recognizing people with and without training videos, and, penalizes methods that are poor at any of the two tasks.  
%Therefore, the task can be summarized learning to
%transfer face recognition models from the domain of clean still images to the domain of violent videos, in a partially
%supervised way. 

We formulate the task as transferring the face recognition model from the domain of clean (so-called \textit{Red Carpet})
images to the domain of violent (\textit{Fight Club}) videos.
% , or \textit{ ``clean-to-violent''} face recognition. 
Since the training videos are labeled but scarce and made available only for a subset of people, we refer to the
learning problem as {\em partially-supervised domain-transfer}.  To tackle this problem, we divide it into two
sub-problems and propose two major techniques for each one.  First, we leverage stacked affine-transform 
layers for classifier transfer, which aims to adapt the image-based classification model to the target-domain
representations, in a supervised yet data-efficient manner. Second, we propose an attention-driven temporal pooling
layer, which aims to enable data-driven adaptation to the face tracks in the video domain. We additionally propose a
third self-attention~\cite{vaswani2017attention} based formulation, with components targeted to both sub-problems.  We rigorously evaluate all
proposed techniques and show their advantages over a number of state-of-the-art alternatives.

To sum up, the contributions of this paper include: 
{\bf (1)} A new dataset called WildestFaces that includes a wide range of examples from violent movies;
{\bf (2)} A new partially-supervised face recognition task, where classifiers trained on clean image data are evaluated for their ability of recognizing faces in violent videos;
{\bf (3)} Rigorous evaluation protocols inspired from the recent developments in related problems (primarily zero-shot learning and few-shot learning);
and {\bf (4)} Effective techniques for the proposed partially-supervised, \textit{clean-to-violent} domain-transfer problem.

%--details of the problem
%--details of the dataset
%--new evaluation protocols
%--benchmark results
%--our new technique

%We provide a detailed discussion of the statistics and the evaluation of state-of-the-art methods on the newly introduced WildestFaces dataset. We exploit the dataset both in the context of video-based face recognition and cross-domain recognition. Our experimental results demonstrate that the state-of-the-art face recognizers fall short for the recognition of faces in the wildest, and there is still a large room for improvement in this challenging dataset that is likely to facilitate further research. 




==> macros.tex <==
% based on Jakob Verbeek's macros.tex

\usepackage{color}
\usepackage[normalem]{ulem}

\def\etal{et al.\ }
\def\Eq#1{Eq.~(\ref{eq:#1})}

\usepackage{amsmath,amssymb,amsbsy,xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eq#1{(\ref{eq:#1})}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}
\def\algo#1{Algorithm~\ref{algo:#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\makeatother

\newcommand{\myparagraphwospace}[1]{\noindent{\bf #1}}
\newcommand{\myparagraphwithspace}[1]{\vspace{6pt}\noindent{\bf #1}} 

